Finding Ethereum Smart Contracts Security Issues by Comparing History Versions

Smart contracts are Turing-complete programs running on the blockchain. They cannot be modified, even when bugs are detected. The Selfdestruct function is the only way to destroy a contract on the blockchain system and transfer all the Ethers on the contract balance. Thus, many developers use this function to destroy a contract and redeploy a new one when bugs are detected. In this paper, we propose a deep learning-based method to find security issues of Ethereum smart contracts by finding the updated version of a destructed contract. After finding the updated versions, we use open card sorting to find security issues.

==> background.tex <==
\section{Background and Motivation}
\label{background}
In this section, we briefly introduce key background information about smart contracts and their contract defects.

\subsection{Smart Contracts}
\noindent {\bf Contracts.}
Leveraging blockchain techniques, smart contracts are autonomous protocols stored on the blockchain. Once started, the running of a contract is automatic and it runs according to the program logic defined beforehand~\cite{chen2018towards}.  When developers deploy a smart contract to Ethereum, the contract will be compiled to EVM bytecode and identified by a unique 160-bit hexadecimal hash contract address. The smart contract execution depends on their code, and even the creator cannot affect its running or state. For example, if a contract does not contain functions for Ether transfer, even the creator cannot withdraw the Ethers. Smart contracts run on a permission-less network. Anyone can invoke the methods of smart contracts through ABI (Application Binary Interface)~\cite{Solidity}. The contract bytecode, transactions, and invocation parameters are visible to everyone.

\noindent {\bf Gas System.}
To ensure the security of smart contracts, each transaction of a smart contract will be run by all miners.  Ethereum uses the \textit{gas system}~\cite{whitepaper} to measure its computational effort, and the developers who send transactions to invoke smart contracts need to pay an execution fee. The execution fee is computed by: $gas\_cost \times gas\_price$. Gas cost depends on the computational resource that takes by the execution and gas price is offered by the transaction creators. To limit gas cost, when developers send their transactions to invoke contracts, they will set the \textit{Gas Limit} which determines the maximum gas cost. If the gas cost of a transaction exceeds its \textit{Gas Limit}, the execution will fail and throw an \emph{out-of-gas error}~\cite{Ethereum_yellow_paper}. There are some special operations which will limit the \textit{Gas Limit} to a specific value. For example, \emph{address.transfer()} and \emph{address.send()} are two methods provided by Ethereum that are used to send Ethers. If a smart contract uses these methods to send Ethers to another smart contract, the \textit{Gas Limit} will be restricted to 2300 gas units~\cite{Solidity}. 2300 gas units are not enough to write to storage, call functions or send Ethers, which can lead to the failure of transactions. Therefore, \emph{address.transfer()} and \emph{address.send()} can only be used to send Ethers to \textit{external owned accounts} (EOA). (There are two types of accounts on Ethereum: externally owned accounts which controlled by private keys, and contract accounts which controlled by their contract code~\cite{Ethereum_yellow_paper}.)


\noindent {\bf Ethereum Virtual Machine (EVM).}
To deploy a smart contract to Ethereum, its source code needs to be compiled to bytecode and stored on the blockchain. EVM is a stack-based machine; when a transaction needs to be executed, EVM will first split bytecode into bytes; each byte represents a unique instruction called opcode. There are 140 unique opcodes by April 2019~\cite{Ethereum_yellow_paper}, and each opcode is represented by a hexadecimal number~\cite{Ethereum_yellow_paper}. EVM uses these opcodes to execute the task. For example, consider a bytecode 0x6070604001. EVM first splits this bytecode into bytes (0x60, 0x70, 0x60, 0x40, 0x01), and execute the first byte 0x60, which refers to opcode \textit{PUSH1}. \textit{PUSH1} pushes one byte data to EVM stack. Therefore, 0x70 is pushed to the stack. Then, EVM reads the next 0x60 and push 0x40 into the stack. Finally, EVM executes 0x01, which refers to opcode \textit{ADD}. \textit{ADD} obtains the next two values from the top of the stack,  i.e., 0x70 and 0x40, and put their sum (B0), a hex result into the stack.

\noindent {\bf The Fallback Function.}
The fallback function is a unique feature of smart contracts compared to traditional programs. An example can be found at Line 13 of Listing 4, which is the only unnamed function in smart contracts programming~\cite{Solidity}. The fallback function does not have any arguments or return values. It will be executed automatically when an error function call happens. For example, if a transaction calls  function `A' of the contract, while there is no function named `A'. In this situation, fallback function will automatically be executed to handle the error call. If the  function is marked by \textit{payable}~\cite{Solidity}, the fallback function will also be executed automatically when receiving Ethers. 

\noindent {\bf The Call Instruction and Ether Transfer.}
Ether transfer is an important feature on Ethereum. In Solidity programming, there are three methods to transfer Ethers, i.e., \textit{address.call.value()}, \textit{address.transfer()}, and \textit{address.send()}. Among these three methods, only \textit{address.call.value()} allows users to send Ethers to a contract address, as the other two methods are limited to 2300 gas units, which are not enough to send Ethers. \textit{address.send()} returns a boolean value, while \textit{address.transfer()} throws an exception when errors happen and returns nothing. All of these three methods can generate a CALL instruction in contract bytecode. Other behaviors, e.g., function call, can also generate CALL instructions. A CALL instruction reads seven values from the top of EVM stack. They represent the gas limitation, recipient address, transfer amount, input data start position, size of the input data,  output data start position, size of the output data, respectively. 


\subsection{Contract Defects in Smart Contracts}
Our previous work \cite{fse-smell} defined 20 contract defects for smart contracts. We divided these contract defects into five ``impact" levels; among these contract defects, 11 belong to impact level one (most serious) to three (low seriousness) that might lead to unwanted behaviors. The definition of these 11 contract defects is given in Table~\ref{tab:difinition}. In this paper, we propose \textit{DefectChecker}, a symbolic execution tool to detect eight of these impact level one to three contract defects. \textit{DefectChecker} does not detect contract defects belonging to levels 4 and 5, as these contract defects will not affect the normal running of the smart contracts according to the definition. For example, \textit{Unspecified Compiler Version} is one of the level 5 smart contract defects. The removal of the contract defects requires the developer of the contract to use a specific compiler like 0.4.25. This contract defect will not affect the normal running of the contract and will only pose a threat for code reuse in the future. This kind of contract defect is also difficult to  detect at the bytecode level as much semantic information is lost after compilation. 

However, please note that in this work, we do not consider three of the contract defects that belong to impact level 1 to 3 -- \textit{Unmatched Type Assignment}, \textit{Hard Code Address} and \textit{Misleading Data Location}, as they are not easy to detect at  bytecode level. Our analysis shows that they appear 22, 84, and 1 times among 587 smart contacts, respectively. EVM will remove or add some information when compiling smart contracts to bytecode, which may cover up these taints on the source contract code. For \textit{\textbf{Hard Code Address}}, the bytecode we obtain from the blockchain does not contain information on the \textit{construct} function, while we found most \textit{Hard Code Address} errors appear in \textit{construct} functions. To detect \textit{\textbf{Unmatched Type Assignment}}, we need to know the maximum loop iterations, which is usually read from storage, and is not easy to obtain the value through static analysis. For example, for a loop ``\textit{for(uint8 i = 0; i $\textless$ num; i++)}", the data range of uint8 is from 0 to 255. Thus, if num is larger than 255, the loop will overflow. However, num is usually a storage variable which is read from storage or depends on an external input. Thus, it is difficult to detect this through bytecode analysis. \textit{\textbf{Misleading Data Location}} is also not easy to detect from bytecode. In Solidity programming, \textit{storage} in Solidity is not dynamically allocated and the type of \textit{struct, array} or \textit{mapping} are maintained on the storage. Thus, these three types created inside a function can point to the \textit{storage slot} 0 by default, which can lead to potential bugs. However, we cannot know whether the point on slot 0 is correct or a mistake made by EVM.  



\begin{table*} 
	%\renewcommand{\arraystretch}{1.1}
	\scriptsize
	\caption{The Definitions of contract defects with Impact level 1-3. The first eight contract defects can be detected by \textit{DefectChecker}.}%\vspace{0.1cm}
	\label{tab:difinition}
	\begin{center}
		\begin{tabular}{p{65pt} | p{140pt} |p{20pt} <{\centering} || p{65pt} | p{140pt} |p{20pt}<{\centering}}
			\hline
			\textbf{Contract Defect} & \textbf{Definition} & \textbf{Impact Level} & \textbf{Contract Defect} & \textbf{Definition} & \textbf{Impact Level}\\
			\hline
			\textit{Transaction State Dependency (TSD)}  & Using tx.origin to check the permission. & IP1  & \textit{DoS Under External Influence (DuEI)}  & Throwing exceptions inside a loop which can be influenced by external users& IP2 \\
			\hline
			\textit{Strict Balance Equality (SBE)}   & Using strict balance quality to determine the execute logic. & IP2 &  \textit{Reentrancy (RE)} & The re-entrancy bugs. & IP1 \\
			\hline
			\textit{Nested Call (NC)}  & Executing CALL instruction inside an unlimited-length loop.& IP2  &  \textit{Greedy Contract (GC)} & A contract can receive Ethers but can not withdraw Ethers. & IP3 \\
			\hline
			\textit{Unchecked External Calls (UEC)} & Do not check the return value of external call functions. & IP3 &   \textit{Block Info Dependency (BID)} & Using block information related functions to determine the execute logic. & IP3 \\
			\hline
			\hline
			\textit{Unmatched Type Assignment} & Assigning unmatched type to a value, which can lead to integer overflow & IP2 & \textit{Misleading Data Location} & The reference types of local variables with \textit{struct}, \textit{array} or \textit{mapping} do not clarify & IP2 \\
			\hline
			\textit{Hard Code Address} & Using hard code address inside smart contracts. & IP3 \\
			\hline
		\end{tabular}
	\end{center}
\end{table*}


\subsubsection{Definition of Impact Levels}

Below we give representative concrete examples of each of the eight smart contract defects, and introduce the definition of impact level one to three according to our previous work.

\begin{itemize}%\setlength{\itemsep}{4pt}
\item \textbf{Impact 1 (IP1):}  Smart contracts containing these contract defects can lead to critical unwanted behaviors. Unwanted behaviors can be triggered by attackers, and they can make profits by utilizing the defects.
\item \textbf{Impact 2 (IP2):} Smart contracts containing these contract defects can lead to critical unwanted behaviors. Unwanted behaviors can be triggered by attackers, but they cannot make profits by utilizing the defects.
\item \textbf{Impact 3 (IP3):} There are two types of IP3. \textbf{Type A}: Smart contracts containing these contract defects can lead to critical unwanted behaviors, but unwanted behaviors cannot be triggered by attackers. \textbf{Type B}: Smart contracts containing these contract defects can lead to major unwanted behaviors. The unwanted behaviors can be triggered by attackers, but they cannot make profits by utilizing the defects.
\end{itemize}	

%According to our previous work. 

Critical represents contract defects, which can lead to the crashing, being controlled by attackers, or can lose all the Ethers. Major represents the contract defects that can lead to the loss of a part of the Ethers ~\cite{fse-smell}.

\subsubsection{Examples of Smart Contract Defects}

\begin{lstlisting}[caption={Transaction State Dependency}]
contract Victim { ...
  address owner = owner_address;
  function sendMoney(address addr){
	require(tx.origin == owner);
	addr.transfer(1 Ether); 
  } 
}
contract Attacker{ ...
  function attack(address vim_addr,address myAddr){
	Victim vic = Victim(vim_addr);
	vic.sendMoney(myAddr);
 }
}
\end{lstlisting} 


\textbf{\textit{(1). Transaction State Dependency (TSD):}} Contracts need to check whether the caller has the right permission for some permission sensitive functions. The failure of the permission check can cause serious consequences. \textit{tx.origin} can get the original address of the transaction, but this method is not reliable as the address returned by this method depends on the transaction state. Therefore, \textit{tx.origin} should not be used to check whether the caller has permission to execute functions.

\textbf{Example}:  In Listing 1, The \textit{Attacker} contract can make a permission check fail by utilizing the \textit{attack} function (Line 9). By utilizing this method, anyone can execute \textit{sendMoney} function (Line 3) and withdraw the Ethers in the contract.

\textbf{Possible Solution}: \textit{Solidity} provides \textit{msg.sender} to obtain the sender address, which can be used to check permissions instead of using \textit{tx.origin}.


\textbf{\textit{(2). DoS under External Influence (DuEI):}} Smart contracts will rollback a transaction if exceptions are detected during their running.  If the error that leads to the exception cannot be fixed, the function will give a denial of service (\textit{DoS}) error perpetually.

\textbf{Example}: Listing 2 shows such an example. Here, \textit{members} is an array which stores many addresses. However, one of the address is an attacker contract, and the transfer function can trigger an out-of-gas exception due to the 2300 gas limitation~\cite{Ethereum_yellow_paper}. Then, the contract state will rollback. Since the code cannot be modified, the contract can not remove the attack address from \textit{members} list, which means that if the attacker does not stop attacking, the following function cannot work anymore.

\textbf{Possible Solution}:  Developers can use a boolean value check instead of throwing exceptions in the loop. For example, using ``\textit{if(members[i].send(0.1 ether) == false) break;}" instead of line 3 in listing 2. 


\begin{lstlisting}[caption={DoS under External Influence}]
for(uint i = 0;i < members.length; i++){
	if(this.balance > 0.1 ether)
		members[i].transfer(0.1 ether); 
}
\end{lstlisting}

\textbf{\textit{(3). Strict Balance Equality (SBE): }}Attackers can send Ethers to any contracts forcibly by utilizing \textit{selfdestruct()}~\cite{Solidity}. This method will not trigger the fallback function, which means the victim contract cannot reject the Ethers. Therefore, smart contract logic may fail to work due to the unexpected Ethers sent by attackers.  

\textbf{Example}:  The \textit{doingSomething()} function in listing 3 can only be triggered when the balance strict equal to 1 \textit{ETH}. However, the attacker can send 1 \textit{Wei} (1 ETH = 1e18 Wei) to the contract to make the balance never equal to 1 ETH.

\textbf{Possible Solution}: The contract can use ``$\geq$" to replace ``==" as attackers can only add to the amount of a balance. In this case, it is difficult for the attackers to affect the logic of the program. 

\begin{lstlisting}[caption={Strict Balance Equality:}]
if(this.balance == 1 eth)  doingSomething();
\end{lstlisting}


\begin{lstlisting}[caption={Reentrancy}]
contract Victim { 	...
  mapping(address => uint) public userBalance;
  function withdraw(){
	uint amount = userBalance[msg.sender];
	if(amount > 0){
	  msg.sender.call.value(amount)();
	  userBalance[msg.sender] = 0; 
	  } 
  } 
  ... 
}
contract Attacker{ 	...
  function() payable{
	Victim(msg.sender).withdraw(); 
  }
  function reentrancy(address addr){
	Victim(addr).withdraw();
  } 
  ...
}
\end{lstlisting}

\textbf{\textit{(4). Reentrancy (RE):}} Ethereum allows parallel external invocations by using the \textit{Call} method. When a contract calls another, the execution waits for the call to finish. The fallback functions of both the callee and caller contract can be executed multiple times during one execution. Thus, it can lead to multiple invocations and money transfer in some situations. 

\textbf{Example}: Listing 4 shows an example of a reentrancy defect. There are two smart contracts, i.e., \textit{Victim} contract and \textit{Attacker} contract. The \textit{Attacker} contract is used to transfer Ethers from \textit{Victim} contract, and the \textit{Victim} contract can be regarded as a bank, which stores the Ethers of users. Users can withdraw their Ethers by invoking \textit{withdraw()} function, which contains Reentrancy defects. 

First, the \textit{Attacker} contract uses the \textit{reentrancy()} function (L16) to invoke \textit{Victim} contract’s \textit{withdraw()} function in line 3. The \textit{addr} in line 16 is the address of the \textit{Victim} contract. Normally, the \textit{Victim} contract sends Ethers to the callee in line 6, and resets callee’s balance to 0 in line 7. However, the \textit{Victim} contract sends Ethers to the \textit{Attacker} contract before resetting the balance to 0. When the \textit{Victim} contract sends Ethers to the \textit{Attacker} contract (L6), the fallback function (L13) of the \textit{Attacker} contract will be invoked automatically, and then invoking the \textit{withdraw()} function (L14) again.  The invoking sequence in this example is: L16 $\rightarrow$ L3 $\rightarrow$ L6 $\rightarrow$ L13 $\rightarrow$  L3 $\rightarrow$ L6 $\rightarrow$ L13 $\cdots$


\textbf{Possible Solution}: There are 3 kinds of \textit{Call} methods that can be used to send Ethers in Ethereum, i.e., \textit{address.send()}, \textit{address.transfer()}, and \textit{address.call.value()}. \textit{address.send()} and  \textit{address.transfer()} will change the maximum gas limitation to 2300 gas units if the recipient is a contract account. 2300 gas units are not enough to transfer Ethers, which means \textit{address.send()} and  \textit{address.transfer()} cannot lead to \textit{Reentrancy}. Therefore, using \textit{address.send()} and  \textit{address.transfer()}  instead \textit{address.call.value()} can avoid \textit{Reentrancy}.

\textbf{\textit{(5). Nested Call (NC):}} Instruction \textit{CALL} is very expensive (9000 gas paid for a non-zero value transfer as part of the CALL operation)~\cite{Ethereum_yellow_paper}. If a loop contains the \textit{CALL} instruction but does not limit the loop iterations,  the total gas cost may have a high risk to exceed its gas limitation.  

\textbf{Example}: In listing 5, if we do not limit the loop iterations, attackers can maliciously increase its size to cause an out-of-gas error.  Once the out-of-gas error happens, this function cannot work anymore, as there is no way to reduce the loop iterations.

\textbf{Possible Solution}: Developers should estimate the maximum loop iterations and limit the loop iterations.


\begin{lstlisting}[caption={Nested Call}]
for(uint i = 0; i < member.length; i++){
	member[i].send(1 wei); 
}
\end{lstlisting}


\textbf{\textit{(6). Greedy Contract (GC):}} Ethers on smart contracts can only be withdrawn by sending Ethers to other accounts or using \textit{selfdestruct} function. Otherwise, even the creators of the smart contracts cannot withdraw the Ethers and Ethers will be locked forever. We define that a contract is a greedy contract if the contract can receive Ethers (contains payable functions) but there is no way to withdraw the Ethers. 

\textbf{Example}: Listing 6 is a greedy contract. The contract is able to receive Ethers as it contains a payable fallback function in line 2. However, the contract does not contain any methods to transfer money to others. Therefore, the Ethers on the contract will be locked forever. 

\textbf{Possible Solution}:  Adding a function to withdraw Ethers if the contract can receive Ethers. 


\begin{lstlisting}[caption={Greedy Contract}]
Contract Greedy{
	function() payable{ 
		process(msg.sender); 
	}
	function process(address addr) {...}
}
\end{lstlisting}

\textbf{\textit{(7). Unchecked External Call (UEC): }}  Solidity provides many functions (\textit{address.send(), address.call()}) to transfer Ethers or call functions between contracts. However, these call-related methods can fail, e.g., have a network error or run out of gas. When errors happen, these functions will return a boolean value but never throw an exception. If the callers do not check the return values of the external calls, they cannot ensure whether the logic of the following code snippets is correct. 

\textbf{Example}: Listing 7 shows such an example. Line 1 does not check the return value of the \textit{address.send()}. As the Ether transfer can sometimes fail, line 1 cannot ensure whether the logic of the following code is correct. 

\textbf{Possible Solution}:  Always checking the return value of the \textit{address.send()} and \textit{address.call()}.
\begin{lstlisting}[caption={Unchecked External Call}]
address.send(ethers); doingSomething();  //bad
if(address.send(ethers)) doingSomething(); //good
\end{lstlisting}


\textbf{\textit{(8). Block Info Dependency (BID):}} Developers can utilize a series of block related functions to obtain block information. For example, block.blockhash is used to obtain the hash number of the current block.  Many smart contracts rely on these functions to decide a program's execution, e.g., generating random numbers.  However, miners can influence block information, e.g, miners can vary the block time stamp by roughly 900 seconds~\cite{oyente}. In this case, the block info dependency operation can be controlled by miners to some extent.

\textbf{Example}: The contract in listing 8 is a code snippet of a roulette contract. The contract utilizes block hash number to select a winner, and send winner one Ether as bonus. However, the miner can control the result. So, the miner can always be the winner. 

\textbf{Possible Solution}: The precondition of a safe random number is that the random number cannot be controlled by a single person, e.g., a miner.  The completely random information we can use in Ethereum includes users' addresses, users' input numbers and so on. Also, it is important to hide the values used by the contract for other players to avoid attacks. Since we cannot hide the address of users and their submitted values on Ethereum, a possible solution to generate random numbers without using block related functions is using a hash number. The algorithm has three rounds:


\textit{Round 1}: Users obtain a random number and generate a hash value in their local machine. The hash value can be obtained by \textit{keccak256} function, which is a function provided by Ethereum. After obtaining the random number, users submit the hash number.

\textit{Round 2}: After all the users submit the hash number, users are required to submit the original random number. The contract checks whether the original number can generate the same hash number by using the same \textit{keccak256} function.

\textit{Round 3}: If all users submit correct original numbers, the contract can use the original numbers to generate a random number.


\begin{lstlisting}[caption={Block Info Dependency: }]
address[] participators;
uint winnerID = uint(block.blockhash) % participators.length
participators[winnerID].transfer(1 eths);
\end{lstlisting}





